Four-dimensional domain decomposition for the factorization of the fermion determinant

The non-local dependence of the fermion determinant on the gauge field limits our ability of simulating Quantum Chromodynamics on the lattice. Here we present a factorization of the gauge field dependence of the fermion determinant based on an overlapping four-dimensional domain decomposition of the lattice. The resulting action is block-local in the gauge and in the auxiliary bosonic fields. Possible applications are multi-level integration, master field simulations, and more efficient parallelizations of Monte Carlo algorithms and codes.

==> appA.tex <==
The massive $O(a)$-improved Wilson-Dirac operator is defined
as\footnote{Throughout this appendix the lattice spacing is set to unity for notational simplicity.}
\cite{Sheikholeslami:1985ij,Luscher:1996sc}
\be\label{eq:Dwimp}
D = D_{\rm w} + D_{\rm sw} + m_{0} \; ,
\ee
where $m_{0}$ is the bare quark mass, $D_{\rm w}$ is the massless Wilson-Dirac operator
\be\label{eq:Dw}
D_{\rm w} = \frac{1}{2} \{ \gamma_{\mu}(\nabla_{\mu}^{*} + \nabla_{\mu} ) - \nabla_{\mu}^{*} \nabla_{\mu} \} \; ,
\ee
with $\gamma_{\mu}$ being the Dirac matrices and the summation over repeated indices is always understood.
The covariant forward and backward derivatives $\nabla_{\mu}$ and $\nabla_{\mu}^{*}$ are defined to be
\be\label{eq:cov}
\nabla_{\mu}\psi(x) = U_{\mu}(x)\psi(x+\hat{\mu})-\psi(x),\;\;\nabla_{\mu}^{*}\psi(x) = \psi(x) - U^{\dagger}_{\mu}(x-\hat{\mu})\psi(x-\hat{\mu})\;,
\ee
where $U_{\mu}(x)$ are the link fields and $\hat{\mu}$ is the unit versor along the direction $\mu$. By inserting
Eq.~(\ref{eq:cov}) in Eq.(\ref{eq:Dw}), the Wilson operator reads
\be\label{DwPsi}
D_{\rm w}\psi(x) = 4\psi(x) - \frac{1}{2} \sum_{\mu=0}^{3} \{ U_{\mu}(x)(1-\gamma_{\mu})\psi(x+\hat{\mu}) + U^{\dagger}_{\mu}(x-\hat{\mu})(1+\gamma_{\mu})\psi(x-\hat{\mu}) \} \; .
\ee
The second term on the r.h.s. of Eq.~(\ref{eq:Dwimp}) is the Sheikholeslami-Wohlert operator defined as 
\be
D_{\rm sw}\psi(x) = c_{_{SW}} \frac{i}{4} \sigma_{\mu\nu} \widehat{F}_{\mu\nu}(x) \psi(x) \; ,
\ee
where $\sigma_{\mu\nu}=\frac{i}{2}[\dirac\mu,\dirac\nu]$, and $\widehat F_{\mu\nu}(x)$ is
the clover discretization of the field strength tensor which is given by
\be
\widehat{F}_{\mu\nu}(x) = \frac{1}{8} \{ Q_{\mu\nu}(x) - Q_{\nu\mu}(x) \}\; , 
\ee
with
\be
\begin{split}
Q_{\mu\nu}(x) &= U_{\mu}(x)\,U_{\nu}(x+\hat{\mu})\,U_{\mu}^{\dagger}(x+\hat{\nu})\,U_{\nu}^{\dagger}(x)
\\ & + U_{\nu}(x)\,U^\dagger_{\mu}(x-\hat{\mu}+\hat{\nu})\,U_{\nu}^{\dagger}(x-\hat{\mu})\,U_{\mu}(x-\hat{\mu})
\\ & + U_{\mu}^{\dagger}(x-\hat{\mu})\,U_{\nu}^{\dagger}(x-\hat{\mu}-\hat{\nu})\,U_{\mu}(x-\hat{\mu}-\hat{\nu})\,U_{\nu}(x-\hat{\nu})
\\ & + U_{\nu}^{\dagger}(x-\hat{\nu})\,U_{\mu}(x-\hat{\nu})\,U_{\nu}(x+\hat{\mu}-\hat{\nu})\,U_{\mu}^{\dagger}(x) \; .
\end{split}
\ee
It is also possible to use the alternative expression for $D_{\rm sw}$ given by
\be
D_{\rm sw} + (4+m_0) \rightarrow (4+m_{0}) \exp{\frac{c_{_{SW}}}{4+m_{0}} \frac{i}{4} \sigma_{\mu\nu} \widehat{F} _{\mu\nu} } \; ,
\ee
which has been proposed in the context of master field simulations~\cite{Francis:2019muy}.

